Progress, Fairness and Justness in Process Algebra

To prove liveness properties of concurrent systems, it is often necessary to postulate progress, fairness and justness properties. This paper investigates how the necessary progress, fairness and justness assumptions can be added to or incorporated in a standard process-algebraic specification formalism. We propose a formalisation that can be applied to a wide range of process algebras. The presented formalism is used to reason about route discovery and packet delivery in the setting of wireless networks.

==> fig/fairness.tex <==
%% Latex Commands%%
\pspicture(-10,-10)(10,10)
\newcommand{\diam}{0.15}
%%  NODES  %%
   \pnode(-0.75,0){i}
   \cnode[linewidth=0.5pt](0,0){\diam}{r}
   \cnode[linewidth=0.5pt](1.5,0){\diam}{s}
   \cnode[linewidth=0.5pt](3,0){\diam}{t}
   \cnode[linewidth=0.5pt](3,0){0.1}{ti}
   %%node names
    \rput(0,-0.3){$r$}
    \rput(1.5,-0.3){$s$}
    \rput(3,-0.3){$t$}

%%  EDGES  %%
\ncline[linewidth=0.5pt,arrowsize=3pt]{->}{i}{r}
\ncline[linewidth=0.5pt,arrowsize=3pt]{->}{r}{s}
\naput[labelsep=1pt,nrot=:U]{\small$a$}
\ncline[linewidth=0.5pt,arrowsize=3pt]{->}{s}{t}
\naput[labelsep=1pt,nrot=:U]{\small$\tau$}
\nccircle[linewidth=0.5pt,arrowsize=3pt]{->}{s}{0.22}
\nbput[labelsep=1pt,npos=0.35,nrot=0]{\small$\tau$}
\endpspicture


==> fig/justness.tex <==
%% Latex Commands%%
\pspicture(-20,-20)(20,20)
\newcommand{\diam}{0.15}

%%%%%diagram 1
%%  NODES  %%
   \pnode(-1.5,0){i1}
   \cnode[linewidth=0.5pt](-0.75,0){\diam}{r1}
   \cnode[linewidth=0.5pt](0.75,0){\diam}{s1}
   \cnode[linewidth=0.5pt](2.25,0){\diam}{t1}
   \cnode[linewidth=0.5pt](2.25,0){0.1}{ti1}
   %%node names
%    \rput(-0.75,-0.3){$r$}
%    \rput(0.75,-0.3){$s$}
%    \rput(2.25,-0.3){$t$}

%%  EDGES  %%
\ncline[linewidth=0.5pt,arrowsize=3pt]{->}{i1}{r1}
\ncline[linewidth=0.5pt,arrowsize=3pt]{->}{r1}{s1}
\naput[labelsep=1pt,nrot=:U]{\small$a$}
\ncline[linewidth=0.5pt,arrowsize=3pt]{->}{s1}{t1}
\naput[labelsep=1pt,nrot=:U]{\small$\tau$}

%%%symbol for parallalism
\rput(3,0){\scalebox{1.5}{$\|$}}

%%%%%diagram 2
\pnode(3.75,0){i2}
\cnode[linewidth=0.5pt](4.5,0){\diam}{r2}
\ncline[linewidth=0.5pt,arrowsize=3pt]{->}{i2}{r2}
\nccircle[linewidth=0.5pt,arrowsize=3pt]{->}{r2}{0.22}
\nbput[labelsep=1pt,npos=0.35,nrot=0]{\small$\tau$}


%%%symbol for equation
\rput(5.55,0){\scalebox{1.5}{$=$}}

%%  NODES  %%
   \pnode(6.25,0){i}
   \cnode[linewidth=0.5pt](7,0){\diam}{r}
   \cnode[linewidth=0.5pt](8.5,0){\diam}{s}
   \cnode[linewidth=0.5pt](10,0){\diam}{t}
   \cnode[linewidth=0.5pt](10,0){0.1}{ti}
   %%node names
    \rput(7,-0.3){$r$}
    \rput(8.5,-0.3){$s$}
    \rput(10,-0.3){$t$}

%%  EDGES  %%
\ncline[linewidth=0.5pt,arrowsize=3pt]{->}{i}{r}
\ncline[linewidth=0.5pt,arrowsize=3pt]{->}{r}{s}
\naput[labelsep=1pt,nrot=:U]{\small$a$}
\ncline[linewidth=0.5pt,arrowsize=3pt]{->}{s}{t}
\naput[labelsep=1pt,nrot=:U]{\small$\tau$}
\nccircle[linewidth=0.5pt,arrowsize=3pt]{->}{r}{0.22}
\nbput[labelsep=1pt,npos=0.35,nrot=0]{\small$\tau$}
\nccircle[linewidth=0.5pt,arrowsize=3pt]{->}{s}{0.22}
\nbput[labelsep=1pt,npos=0.35,nrot=0]{\small$\tau$}
\nccircle[linewidth=0.5pt,arrowsize=3pt]{->}{t}{0.22}
\nbput[labelsep=1pt,npos=0.35,nrot=0]{\small$\tau$}
\endpspicture


==> fig/progress.tex <==
%% Latex Commands%%
\pspicture(-10,-10)(10,10)
\newcommand{\diam}{0.15}
%%  NODES  %%
   \pnode(-0.75,0){i}
   \cnode[linewidth=0.5pt](0,0){\diam}{r}
   \cnode[linewidth=0.5pt](1.5,0){\diam}{s}
   \cnode[linewidth=0.5pt](3,0){\diam}{t}
   \cnode[linewidth=0.5pt](3,0){0.1}{ti}
   %%node names
    \rput(0,-0.3){$r$}
    \rput(1.5,-0.3){$s$}
    \rput(3,-0.3){$t$}

%%  EDGES  %%
\ncline[linewidth=0.5pt,arrowsize=3pt]{->}{i}{r}
\ncline[linewidth=0.5pt,arrowsize=3pt]{->}{r}{s}
\naput[labelsep=1pt,nrot=:U]{\small$a$}
\ncline[linewidth=0.5pt,arrowsize=3pt]{->}{s}{t}
\naput[labelsep=1pt,nrot=:U]{\small$\tau$}

\endpspicture

